Constrained Adaptive Attacks: Realistic Evaluation of Adversarial Examples and Robust Training of Deep Neural Networks for Tabular Data

State-of-the-art deep learning models for tabular data have recently achieved acceptable performance to be deployed in industrial settings. However, the robustness of these models remains scarcely explored. Contrary to computer vision, there is to date no realistic protocol to properly evaluate the adversarial robustness of deep tabular models due to intrinsic properties of tabular data such as categorical features, immutability, and feature relationship constraints. To fill this gap, we propose CAA, the first efficient evasion attack for constrained tabular deep learning models. CAA is an iterative parameter-free attack that combines gradient and search attacks to generate adversarial examples under constraints. We leverage CAA to build a benchmark of deep tabular models across three popular use cases: credit scoring, phishing and botnet attacks detection. Our benchmark supports ten threat models with increasing capabilities of the attacker, and reflects real-world attack scenarios for each use case. Overall, our results demonstrate how domain knowledge, adversarial training, and attack budgets impact the robustness assessment of deep tabular models and provide security practitioners with a set of recommendations to improve the robustness of deep tabular models against various evasion attack scenarios.

==> pages/5.1-scenarioA.tex <==
\paragraph{Effectiveness and efficiency of the attacks}

We compare the robust accuracy after each of the constrained attacks CPGD, CAPGD, MOEVA and CAA for on the standard and robust models across all our datasets in figure \ref{fig:scenario_a_effectiveness} (and detailed results in Appendix B). Against non-robust models (dashed lines), CAA with domain knowledge outperforms all the attacks in 6 over 9 cases. It is the equally performing as the best attack (MOEVA) in the three remaining cases of CTU. 
%
Against adversarially trained models (continuous lines), CAA and MOEVA achieve similar performances across all our datasets and models.

CAA particularly shines in terms of efficiency. It is always less expensive than MOEVA. The cost of attacking standard URL models is divided by three for TabTransformer and RLN and by five for a standard RLN model on the LCLD dataset.  

\paragraph{Impact of domain-knowledge}

We compare in figure \ref{fig:scenario_a_effectiveness} how access to domain-knowledge (scenario A1 in blue) significantly impact the attacker's ability to attack the ML system. Except for TabTransformer model on CTU dataset, attackers with domain knowledge significantly outperform attackers without. URL dataset has the simplest domain constraints and both attacks with and without domain knowledge on undefended models lead to low robust accuracies, while it is impossible to attack a model on LCLD dataset without domain knowledge. On the CTU dataset, with the largest number of domain constraints, it is only possible to attack the models when the constraints are known and the model undefended. 

Robust models (continuous lines) reduce the gap between attacks that have access to domain knowledge and attacks that don't. It is consistent across our 9 cases and confirms that local robustness archived by adversarial training hinders label flips under satisfaction of the constraints. Our detailed results in appendix B show that adversarial training reduces both the misclassification and the constraint satisfaction in an epsilon-bounded perturbation. 

\paragraph{Impact of architecture}

For each dataset, the test performances of the three architectures are equivalent (Standard in figure \ref{fig:scenario_a_effectiveness}), however their robustness can significantly vary.
On the simplest dataset, URL, VIME (Data transformation family) is particularly robust, even without adversarial training. On the most complex dataset, CTU, Tabtransformer (Architecture optimisation family) is unperturbed by adversarial examples, while VIME is particularly weak without adversarial training.

Our results also demonstrate that all architectures that are vulnerable to adversarial examples significantly benefit from adversarial training, especially RLN (regularization family).  



\paragraph{Impact of budget}

We compare in table \ref{fig:scenario_a_budget} the impact of changing the $epislon$ budget of the CAA attack with domain knowledge (A1) from 0.5 to 0.25 and to 1. The conclusions remain valid with the remaining whitebox attacks and in scenario A2 (cf appendix ...).

For models with standard training, increasing the budget of attacks completely breaks the robustness of the models for all architectures on URL and LCLD datasets. Adversarialy trained models are also significantly impact for URL dataset and marginally impacted for LCLD. 

Across all our models for CTU, increasing the $\epsilon$ budget of the attack has negeligeable impact on the robustness of models. 


\begin{table*}
\centering
\caption{Adversarial robustness against CAA attacks with increasing $\epsilon$ budgets for scenario A1 (Cstr: Yes) and A2 (Cstr: False)}
 \label{fig:scenario_a_budget}
\footnotesize
\begin{tabular}{lll|lllllllll}
\toprule
        Dataset&    & & \multicolumn{3}{c}{URL} & \multicolumn{3}{c}{LCLD} & \multicolumn{3}{c}{CTU} \\
        Model&    & &                        RLN &                  TabTrans. &                       VIME &                        RLN &                  TabTrans. &                       VIME &                        RLN &                  TabTrans. &                       VIME \\
Training & Cstr & $\epsilon$ &                            &                            &                            &                            &                            &                            &                            &                            &                            \\
\midrule
\multirow{6}{*}{Standard} & \multirow{3}{*}{Yes} & 0.25 &  $0.366$\tiny{$\pm 0.004$} &  $0.315$\tiny{$\pm 0.001$} &  $0.697$\tiny{$\pm 0.003$} &  $0.002$\tiny{$\pm 0.000$} &  $0.273$\tiny{$\pm 0.003$} &  $0.224$\tiny{$\pm 0.002$} &  $0.952$\tiny{$\pm 0.003$} &  $0.953$\tiny{$\pm 0.000$} &  $0.561$\tiny{$\pm 0.034$} \\
       &    & 0.5 &  $0.123$\tiny{$\pm 0.006$} &  $0.088$\tiny{$\pm 0.002$} &  $0.492$\tiny{$\pm 0.005$} &  $0.001$\tiny{$\pm 0.001$} &  $0.135$\tiny{$\pm 0.006$} &  $0.066$\tiny{$\pm 0.005$} &  $0.940$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} \\
       &    & 1.0 &  $0.115$\tiny{$\pm 0.006$} &  $0.014$\tiny{$\pm 0.001$} &  $0.161$\tiny{$\pm 0.004$} &  $0.000$\tiny{$\pm 0.000$} &  $0.080$\tiny{$\pm 0.005$} &  $0.022$\tiny{$\pm 0.004$} &  $0.940$\tiny{$\pm 0.002$} &  $0.951$\tiny{$\pm 0.002$} &  $0.340$\tiny{$\pm 0.040$} \\
\cline{2-12}
       & \multirow{3}{*}{No} & 0.25 &  $0.371$\tiny{$\pm 0.003$} &  $0.316$\tiny{$\pm 0.004$} &  $0.696$\tiny{$\pm 0.005$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.976$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
       &    & 0.5 &  $0.224$\tiny{$\pm 0.003$} &  $0.131$\tiny{$\pm 0.006$} &  $0.499$\tiny{$\pm 0.004$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
       &    & 1.0 &  $0.220$\tiny{$\pm 0.005$} &  $0.142$\tiny{$\pm 0.008$} &  $0.168$\tiny{$\pm 0.007$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
\cline{1-12}
\cline{2-12}
\multirow{6}{*}{Robust} & \multirow{3}{*}{Yes} & 0.25 &  $0.832$\tiny{$\pm 0.002$} &  $0.830$\tiny{$\pm 0.002$} &  $0.827$\tiny{$\pm 0.002$} &  $0.672$\tiny{$\pm 0.002$} &  $0.719$\tiny{$\pm 0.002$} &  $0.302$\tiny{$\pm 0.003$} &  $0.971$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} \\
       &    & 0.5 &  $0.562$\tiny{$\pm 0.006$} &  $0.567$\tiny{$\pm 0.008$} &  $0.697$\tiny{$\pm 0.006$} &  $0.661$\tiny{$\pm 0.003$} &  $0.708$\tiny{$\pm 0.002$} &  $0.147$\tiny{$\pm 0.005$} &  $0.971$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} \\
       &    & 1.0 &  $0.223$\tiny{$\pm 0.009$} &  $0.252$\tiny{$\pm 0.022$} &  $0.272$\tiny{$\pm 0.008$} &  $0.656$\tiny{$\pm 0.003$} &  $0.692$\tiny{$\pm 0.003$} &  $0.104$\tiny{$\pm 0.003$} &  $0.971$\tiny{$\pm 0.000$} &  $0.952$\tiny{$\pm 0.002$} &  $0.910$\tiny{$\pm 0.017$} \\
\cline{2-12}
       & \multirow{3}{*}{No} & 0.25 &  $0.831$\tiny{$\pm 0.002$} &  $0.832$\tiny{$\pm 0.001$} &  $0.827$\tiny{$\pm 0.002$} &  $0.691$\tiny{$\pm 0.001$} &  $0.744$\tiny{$\pm 0.000$} &  $0.626$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} \\
       &    & 0.5 &  $0.559$\tiny{$\pm 0.005$} &  $0.570$\tiny{$\pm 0.008$} &  $0.699$\tiny{$\pm 0.003$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.623$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} \\
       &    & 1.0 &  $0.213$\tiny{$\pm 0.006$} &  $0.258$\tiny{$\pm 0.026$} &  $0.282$\tiny{$\pm 0.010$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.622$\tiny{$\pm 0.002$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.921$\tiny{$\pm 0.015$} \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}
 \label{fig:scenario_a_budget_steps_main}
\centering
\caption{Robust accuracy with different \#step for CAA attack.}
\footnotesize
\begin{tabular}{lll|lllllllll}
\toprule
        Dataset&    & & \multicolumn{3}{c}{URL} & \multicolumn{3}{c}{LCLD} & \multicolumn{3}{c}{CTU} \\
         Model&    & &                        RLN &                  TabTrans. &                       VIME &                        RLN &                  TabTrans. &                       VIME &                        RLN &                  TabTrans. &                       VIME \\
Training & Cstr & Stp &                            &                            &                            &                            &                            &                            &                            &                            &                            \\
\midrule
\multirow{8}{*}{Standard} & \multirow{4}{*}{Yes} & 10  &  $0.123$\tiny{$\pm 0.006$} &  $0.088$\tiny{$\pm 0.002$} &  $0.492$\tiny{$\pm 0.005$} &  $0.001$\tiny{$\pm 0.001$} &  $0.135$\tiny{$\pm 0.006$} &  $0.066$\tiny{$\pm 0.005$} &  $0.940$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} \\
       &    & 20  &  $0.086$\tiny{$\pm 0.003$} &  $0.079$\tiny{$\pm 0.000$} &  $0.470$\tiny{$\pm 0.003$} &  $0.000$\tiny{$\pm 0.000$} &  $0.132$\tiny{$\pm 0.003$} &  $0.056$\tiny{$\pm 0.003$} &  $0.940$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} \\
       &    & 50  &  $0.091$\tiny{$\pm 0.003$} &  $0.087$\tiny{$\pm 0.002$} &  $0.463$\tiny{$\pm 0.003$} &  $0.000$\tiny{$\pm 0.000$} &  $0.120$\tiny{$\pm 0.005$} &  $0.042$\tiny{$\pm 0.004$} &  $0.940$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} \\
       &    & 100 &  $0.087$\tiny{$\pm 0.002$} &  $0.084$\tiny{$\pm 0.001$} &  $0.459$\tiny{$\pm 0.002$} &  $0.000$\tiny{$\pm 0.000$} &  $0.114$\tiny{$\pm 0.005$} &  $0.033$\tiny{$\pm 0.001$} &  $0.940$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} \\
\cline{2-12}
       & \multirow{4}{*}{No} & 10  &  $0.224$\tiny{$\pm 0.003$} &  $0.131$\tiny{$\pm 0.006$} &  $0.499$\tiny{$\pm 0.004$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
       &    & 20  &  $0.224$\tiny{$\pm 0.005$} &  $0.132$\tiny{$\pm 0.006$} &  $0.479$\tiny{$\pm 0.003$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
       &    & 50  &  $0.223$\tiny{$\pm 0.004$} &  $0.134$\tiny{$\pm 0.007$} &  $0.474$\tiny{$\pm 0.003$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
       &    & 100 &  $0.222$\tiny{$\pm 0.005$} &  $0.132$\tiny{$\pm 0.007$} &  $0.469$\tiny{$\pm 0.004$} &  $0.542$\tiny{$\pm 0.008$} &  $0.671$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} &  $0.953$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} \\
\cline{1-12}
\cline{2-12}
\multirow{8}{*}{Robust} & \multirow{4}{*}{Yes} & 10  &  $0.562$\tiny{$\pm 0.006$} &  $0.567$\tiny{$\pm 0.008$} &  $0.697$\tiny{$\pm 0.006$} &  $0.661$\tiny{$\pm 0.003$} &  $0.708$\tiny{$\pm 0.002$} &  $0.147$\tiny{$\pm 0.005$} &  $0.971$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} \\
       &    & 20  &  $0.562$\tiny{$\pm 0.006$} &  $0.567$\tiny{$\pm 0.008$} &  $0.696$\tiny{$\pm 0.006$} &  $0.660$\tiny{$\pm 0.003$} &  $0.706$\tiny{$\pm 0.001$} &  $0.132$\tiny{$\pm 0.007$} &  $0.971$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} \\
       &    & 50  &  $0.562$\tiny{$\pm 0.006$} &  $0.567$\tiny{$\pm 0.009$} &  $0.696$\tiny{$\pm 0.006$} &  $0.656$\tiny{$\pm 0.003$} &  $0.705$\tiny{$\pm 0.003$} &  $0.135$\tiny{$\pm 0.006$} &  $0.971$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} \\
       &    & 100 &  $0.562$\tiny{$\pm 0.006$} &  $0.567$\tiny{$\pm 0.008$} &  $0.696$\tiny{$\pm 0.006$} &  $0.653$\tiny{$\pm 0.001$} &  $0.703$\tiny{$\pm 0.003$} &  $0.129$\tiny{$\pm 0.005$} &  $0.971$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} \\
\cline{2-12}
       & \multirow{4}{*}{No} & 10  &  $0.559$\tiny{$\pm 0.005$} &  $0.570$\tiny{$\pm 0.008$} &  $0.699$\tiny{$\pm 0.003$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.623$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} \\
       &    & 20  &  $0.559$\tiny{$\pm 0.005$} &  $0.569$\tiny{$\pm 0.007$} &  $0.698$\tiny{$\pm 0.004$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.623$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} \\
       &    & 50  &  $0.559$\tiny{$\pm 0.004$} &  $0.570$\tiny{$\pm 0.008$} &  $0.698$\tiny{$\pm 0.003$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.623$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} \\
       &    & 100 &  $0.559$\tiny{$\pm 0.004$} &  $0.570$\tiny{$\pm 0.008$} &  $0.697$\tiny{$\pm 0.003$} &  $0.690$\tiny{$\pm 0.002$} &  $0.743$\tiny{$\pm 0.001$} &  $0.623$\tiny{$\pm 0.003$} &  $0.972$\tiny{$\pm 0.001$} &  $0.953$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} \\
\bottomrule
\end{tabular}

\end{table*}

==> pages/5.2-scenarioB.tex <==
In the query-based scenario, the critical property is the number of queries needed by the attacker. In MOEVA, a genetic algorithm, it is the product of the number of search generation and the number of offspring at each generation. We evaluate the models trained on the LCLD, URL, and CTU datasets in 
%figure \ref{fig:scenario_b_cost_lcld}, figure \ref{fig:scenario_b_cost_url}, and figure \ref{fig:scenario_b_cost_ctu} 
table \ref{tab:scenario_b_cost} 
the robust accuracy of each of the standard (a) and adversarialy trained models (b) with increased budgets of MOEVA.

Across all our LCLD models%(figure \ref{fig:scenario_b_cost_lcld})
, increasing the budget of the attack does not significantly impact its effectiveness. Robust models (adversarially trained RLN and TabTransformer) remain robust under four times budget increase.

The robustness of models trained on the URL dataset %(figure \ref{fig:scenario_b_cost_url}) 
on the contrary is very sensitive to the attack budgets, and for all models drops with increased generations or offspring. For robust RLN and Tabtransformer the accuracy is halved when the budget is quadrupled. None of the architecture with standard training remains robust with increased budgets, with the robust accuracy dropping as low as 0.056 for Tabtransformer.

Models trained on CTU %(figure \ref{fig:scenario_b_cost_ctu}) 
exhibit an intermediary scenario. While robust CTU models are not impacted by an increased budget, RLN and VIME models trained without adversarial training see their robust accuracy collapses to 0.01 with quadrupled budget. TabTransformer models remain robust with standard training even under increased budgets. 




\begin{table*}[]
\centering
\caption{Model robustness in the scenarios B1 for our three datasets. The budget is (\#generation)x(\#offspring per generation).}
\label{tab:scenario_b_cost}
\footnotesize

\begin{tabular}{@{}ll|lllllllll@{}}
\toprule
Dataset &       & \multicolumn{3}{c}{URL}                                                              & \multicolumn{3}{c}{LCLD}                                                             & \multicolumn{3}{c}{CTU}                                                              \\
Model        &         & RLN                        & TabTrans.             & VIME                       & RLN                        & TabTrans.             & VIME                       & RLN                        & TabTrans.             & VIME                       \\
Training            & Budget  &                            &                            &                            &                            &                            &                            &                            &                            &                            \\ \midrule
\multirow{5}{*}{Standard} & 50x50   & $0.612$\tiny{$\pm 0.009$} & $0.577$\tiny{$\pm 0.003$} & $0.785$\tiny{$\pm 0.009$} & $0.017$\tiny{$\pm 0.007$} & $0.258$\tiny{$\pm 0.005$} & $0.281$\tiny{$\pm 0.009$} & $0.964$\tiny{$\pm 0.001$} & $0.953$\tiny{$\pm 0.000$} & $0.888$\tiny{$\pm 0.016$} \\
                          & 100x100 & $0.236$\tiny{$\pm 0.005$} & $0.182$\tiny{$\pm 0.008$} & $0.565$\tiny{$\pm 0.009$} & $0.006$\tiny{$\pm 0.002$} & $0.150$\tiny{$\pm 0.007$} & $0.269$\tiny{$\pm 0.018$} & $0.940$\tiny{$\pm 0.002$} & $0.953$\tiny{$\pm 0.000$} & $0.408$\tiny{$\pm 0.047$} \\
                          & 100x200 & $0.162$\tiny{$\pm 0.003$} & $0.093$\tiny{$\pm 0.006$} & $0.368$\tiny{$\pm 0.010$} & $0.042$\tiny{$\pm 0.007$} & $0.160$\tiny{$\pm 0.006$} & $0.308$\tiny{$\pm 0.020$} & $0.303$\tiny{$\pm 0.066$} & $0.953$\tiny{$\pm 0.000$} & $0.088$\tiny{$\pm 0.018$} \\
                          & 200x100 & $0.154$\tiny{$\pm 0.002$} & $0.087$\tiny{$\pm 0.002$} & $0.353$\tiny{$\pm 0.004$} & $0.053$\tiny{$\pm 0.006$} & $0.169$\tiny{$\pm 0.007$} & $0.315$\tiny{$\pm 0.015$} & $0.241$\tiny{$\pm 0.061$} & $0.953$\tiny{$\pm 0.000$} & $0.060$\tiny{$\pm 0.015$} \\
                          & 200x200 & $0.134$\tiny{$\pm 0.005$} & $0.056$\tiny{$\pm 0.003$} & $0.293$\tiny{$\pm 0.002$} & $0.076$\tiny{$\pm 0.011$} & $0.179$\tiny{$\pm 0.007$} & $0.332$\tiny{$\pm 0.012$} & $0.010$\tiny{$\pm 0.002$} & $0.953$\tiny{$\pm 0.000$} & $0.013$\tiny{$\pm 0.001$} \\ \midrule
\multirow{5}{*}{Robust}   & 50x50   & $0.834$\tiny{$\pm 0.009$} & $0.827$\tiny{$\pm 0.012$} & $0.836$\tiny{$\pm 0.006$} & $0.673$\tiny{$\pm 0.002$} & $0.717$\tiny{$\pm 0.001$} & $0.314$\tiny{$\pm 0.011$} & $0.972$\tiny{$\pm 0.001$} & $0.953$\tiny{$\pm 0.000$} & $0.949$\tiny{$\pm 0.002$} \\
                          & 100x100 & $0.563$\tiny{$\pm 0.007$} & $0.568$\tiny{$\pm 0.008$} & $0.700$\tiny{$\pm 0.006$} & $0.662$\tiny{$\pm 0.002$} & $0.713$\tiny{$\pm 0.002$} & $0.226$\tiny{$\pm 0.008$} & $0.971$\tiny{$\pm 0.000$} & $0.953$\tiny{$\pm 0.000$} & $0.940$\tiny{$\pm 0.005$} \\
                          & 100x200 & $0.431$\tiny{$\pm 0.003$} & $0.445$\tiny{$\pm 0.002$} & $0.620$\tiny{$\pm 0.005$} & $0.663$\tiny{$\pm 0.003$} & $0.715$\tiny{$\pm 0.002$} & $0.240$\tiny{$\pm 0.010$} & $0.970$\tiny{$\pm 0.001$} & $0.953$\tiny{$\pm 0.000$} & $0.928$\tiny{$\pm 0.004$} \\
                          & 200x100 & $0.424$\tiny{$\pm 0.001$} & $0.441$\tiny{$\pm 0.003$} & $0.613$\tiny{$\pm 0.005$} & $0.664$\tiny{$\pm 0.001$} & $0.715$\tiny{$\pm 0.002$} & $0.247$\tiny{$\pm 0.008$} & $0.969$\tiny{$\pm 0.001$} & $0.953$\tiny{$\pm 0.000$} & $0.924$\tiny{$\pm 0.005$} \\
                          & 200x200 & $0.403$\tiny{$\pm 0.001$} & $0.415$\tiny{$\pm 0.002$} & $0.589$\tiny{$\pm 0.007$} & $0.664$\tiny{$\pm 0.002$} & $0.714$\tiny{$\pm 0.002$} & $0.249$\tiny{$\pm 0.009$} & $0.968$\tiny{$\pm 0.000$} & $0.953$\tiny{$\pm 0.000$} & $0.907$\tiny{$\pm 0.005$} \\ \bottomrule
\end{tabular}
\end{table*}

==> pages/5.3-scenarioCDE.tex <==
\paragraph{Impact of architecture}

We first compare in table \ref{tab:surrogate_ranking_main} the ranking of each architecture in terms of robust accuracy when used as a surrogate source model (by the attacker), and when used as target (the defender) for each of our scenarios: Where the surrogate has access to the full training set (C1), a subset of the training set (D1) and only a knowledge of the training distribution (E1).

The lower the rank the best for the attacker, and the higher the rank the better for the defender.

Our results show that for robust targets TabTransformer is the best architecture for the defender, and VIME the worst. There is however no architecture that is reliably best suited to use as a surrogate source against standard and robust targets.


\begin{table}
\small
    \centering
    \caption{Rank of target robust accuracy when using different architectures as source with standard training (the lowest rank best for attacker), and as target (the highest rank the best for defender) }
    \begin{tabular}{c|c|lll|lll}
Target              &                & \multicolumn{3}{c|}{As a source $\downarrow$}                                          & \multicolumn{3}{c}{As a target $\uparrow$  }                                          \\ \hline
Standard & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
                & Transformer & 1.5                    & 2                      & 2                       & 1                      & 2                      & 1.5                    \\
                & RLN            & 1.5                    & 1                      & 1                       & 1.5                    & 1                      & 1                      \\
                & VIME           & 1.5                    & 1.5                    & 1.5                     & 2                      & 1.5                    & 2                      \\ \hline
Robust   & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
                & Transformer & 1.5                    & 2                      & 1.5                     & 2                      & 2                      & 2                      \\
                & RLN            & 1.5                    & 1.5                    & 1                       & 1.5                    & 1.5                    & 1.5                    \\
                & VIME           & 1.5                    & 1                      & 2                       & 1                      & 1                      & 1                     
\end{tabular}
    
    \label{tab:surrogate_ranking_main}
\end{table}




\paragraph{Impact of domain knowledge}

Next, we compare in figure \ref{fig:scenario_cde_lcld} the effectiveness of surrogate attacks under our three scenarios. For each case, we assess the effectiveness of the attacks when the domain constraints are known (left figures) or unavailable (right figures). We also compare the scenarios where the target models have been robustified (bottom) or not (top). 

For each target model, we use the remaining models as surrogates and report the interval of robust accuracy between the worst and the best surrogate model (colored area). 

When the models are not robustified (top), There is a significant variance in the effectiveness of the surrogate model when the attacker has a full knowledge of domain (scenarios C1, D1, E1) compared to attackers with no domain knowledge (C2, D2, E2). The latter are impossible to attack when we move from whitebox (A2) to the remaining graybox scenarios (C2, D2, E2).   


\paragraph{Impact of adversarial training}
Similarly, the variance in the effectiveness of the surrogates models decreases significantly when target model is robustified (bottom) for TabTransformer and RLN. However, the variance of VIME models with and without adversarial training for scenario D1 is high. 

\paragraph{Impact of attack scenario}

Surprisingly, attacking a standard Tabtransformer model is more effective when the surrogate only has access to the training distribution (E1) instead of the actual training dataset (C1). In all the other cases, having access to the training set does not bring any advantage to the attacker over knowing the training distribution of the target.  



\begin{figure*}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/lcld_v2_iid/acde_Standard_1.pdf}
    \caption{Standard target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/lcld_v2_iid/acde_Standard_2.pdf}
    \caption{Standard target (A2, C2, D2, E2)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/lcld_v2_iid/acde_Robust_1.pdf}
    \caption{Robust target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/lcld_v2_iid/acde_Robust_2.pdf}
    \caption{Robust target (A2, C2, D2, E2)}
    \end{subfigure}

    \caption{Robust accuracy for different scenarios and target models. C1/C2 source is not robust. The range represents the min-max interval, over 5 seeds for A, and over 5 seeds and 2 source models (different from the target model) for C D E.}
    \label{fig:scenario_cde_lcld}
\end{figure*}








==> pages/6-qualitative.tex <==
\section{Qualitative analysis of the adversarial examples}

In the following we study for the LCLD dataset how are the adversarial examples generated against a TabTransformer model in the A1 scenario. We first explore the feature perturbations, then study the constraints violations. We focus on LCLD for its diversity of constraints and high success rate of CAA in A1 scenario.

\paragraph{Feature Perturbations}

\begin{figure}[]
\centering
  \includegraphics[width=\linewidth]{figures/rotten_tomatoes_clean_both_embd_class_1.png}
  \caption{PLACEHOLDER: t-SNE visualization of original examples and the successful adversarial examples generated by DeepWordBug and TextFooler for Rotten Tomatoes positive reviews.}
  \label{fig-text-rq3}
  \end{figure}

\paragraph{Constraints Violations}

\begin{table}
\centering
\caption{Constraints satisfcation after each of the attacks}
\begin{tabular}{ll|lll}
\toprule
           & Attack &             CPGD & CAPGD & MOEVA \\
Constraint & Type &                  &       &       \\
\midrule
$\phi_{1}$ & $\land, \leq$ &            0.265 & 0.863 & 0.904 \\
$\phi_{2}$ & $\leq$ &            0.268 & 0.898 & 0.928 \\
$\phi_{3}$ & $\leq$ &            0.268 & 0.898 & 0.928 \\
$\phi_{4}$ & $\in$ &            0.268 & 0.898 & 0.928 \\
$\phi_{5}$ & $=$ &            0.268 & 0.898 & 0.301 \\
$\phi_{6}$ & $=$ &            0.268 & 0.898 & 0.079 \\
$\phi_{7}$ & $=$ &            0.268 & 0.898 & 0.928 \\
$\phi_{8}$ & $=$ &            0.268 & 0.898 & 0.928 \\
$\phi_{9}$ & $=$ &            0.268 & 0.898 & 0.928 \\
\bottomrule
\end{tabular}
\end{table}


==> pages/7-takeaways.tex <==
\section{Takeaways}

Following our extensive analysis, we draw the following recommendations for tabular machine learning practitioners:

%\paragraph{For attackers}

\paragraph{Threat models.} When the white-box setting is possible, combining gradient and search attacks in our attack CAA significantly speeds up the attack. CAA even remains effective in transfer setting against some robustified models. In the query setting, increasing the budget can significantly break the robustness of models in some datasets. 

\paragraph{Domain knowledge.} The domain-specific constraints of the model are the ultimate defense against adversarial attacks. It is the only mechanism that consistently leads to high robustness across all the threat models, and when broken by the attacker (scenarios A1, B1, ...) leads to the collapse of the robustness of the models.

\paragraph{Architecture selection.} Even if the SotA models in the literature seem to achieve similar test performance, they exhibit large differences in their robustness. VIME is consistently weak across the threat models compared to TabTransformer and RLN.  
%Which architecture is best to attack?

\paragraph{Dataset privacy.} Building a surrogate from data of the same distribution as the target, without accessing the actual training is sufficient to attack both standard and adversarial trained models. Assuming that the training data is inaccessible for the attacker is therefore a weak assumption for a reliable defense. 

\paragraph{Adversarial training.} Gradient-based robustification is very effective as well as against white-box gradient attacks, as against query-based and surrogate-based attacks. It remains effective even when the attacker has access to the training distribution, when the training data of the target model is leaked or when the attacker increases the attack budget (up to 4 times in our study).




==> pages/a-additional-datasets.tex <==


\section{Additional dataset results}

This section presents additional results for URL and CTU datasets.
\subsection{Model ranking}


\begin{table}[h]
\small
    \centering
 \begin{tabular}{c|c|lll|lll}
                \toprule
              &                & \multicolumn{3}{c|}{As a source $\downarrow$}                                          & \multicolumn{3}{c}{As a target $\uparrow$  }                                          \\ 
 & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
%\clin
Target              &       Model  & & & & & & \\ \midrule
                & TabTransf. & 1                      & 1                      & 1                       & 1                      & 1                      & 1                      \\
                & RLN            & 1.5                    & 2                      & 1.5                     & 1.5                    & 1.5                    & 1.5                    \\
                & VIME           & 2                      & 1.5                    & 2                       & 2                      & 2                      & 2                      \\ \midrule
% Robust target   & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
                & TabTransf. & 1.5                    & 1                      & 1.5                     & 1                      & 1                      & 1                      \\
                & RLN            & 1                      & 1.5                    & 1.5                     & 1.5                    & 2                      & 2                      \\
                & VIME           & 2                      & 2                      & 1.5                     & 2                      & 1.5                    & 1.5                   \\ \bottomrule
\end{tabular}
    \caption{URL - Rank of target robust accuracy when using different architectures as source with standard training (the lowest rank best for attacker), and as target (the highest rank the best for defender) }
    \label{tab:surrogate_ranking_url}
\end{table}


\begin{table}[h]
\small
\centering
 \begin{tabular}{c|c|lll|lll}
    \toprule
              &                & \multicolumn{3}{c|}{As a source $\downarrow$}                                          & \multicolumn{3}{c}{As a target $\uparrow$  }                                          \\ 
 & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
%\clin
Target              &       Model  & & & & & & \\ \midrule
Standard                & TabTransf. & 1.5                    & 1.5                    & 1.5                     & 1.5                    & 1.5                    & 1.5                    \\
                & RLN            & 1.5                    & 1.5                    & 1.5                     & 2                      & 2                      & 2                      \\
                & VIME           & 1.5                    & 1.5                    & 1.5                     & 1                      & 1                      & 1                      \\ \midrule
% Robust    & Scenario       & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c|}{E1} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{E1} \\
Robust              & TabTransf. & 1.5                    & 1.5                    & 1.5                     & 1.5                    & 1.5                    & 1.5                    \\
                & RLN            & 1.5                    & 1.5                    & 1.5                     & 2                      & 2                      & 2                      \\
                & VIME           & 1.5                    & 1.5                    & 1.5                     & 1                      & 1                      & 1                     \\ \bottomrule
\end{tabular}
    \caption{CTU - Rank of target robust accuracy when using different architectures as source with standard training (the lowest rank best for attacker), and as target (the highest rank the best for defender) }
    \label{tab:surrogate_ranking_ctu}
\end{table}

Table \ref{tab:surrogate_ranking_url} and \ref{tab:surrogate_ranking_ctu} compares the model architectures in attacker and defender settings for URL and CTU datasets respectively.



\subsection{Scenario A/C/D/E with (1) and without (2) constraints access}


\begin{figure*}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/url/acde_Standard_1.pdf}
    \caption{Standard target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/url/acde_Standard_2.pdf}
    \caption{Standard target (A2, C2, D2, E2)}
    \end{subfigure}

    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/url/acde_Robust_1.pdf}
    \caption{Robust target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/url/acde_Robust_2.pdf}
    \caption{Robust target (A2, C2, D2, E2)}
    \end{subfigure}

    \caption{URL - Robust accuracy for different scenarios and target models. C1/C2 source is not robust. The range represents the 95\% confidence interval, over 5 seeds for A, and over 5 seeds and 2 source models (different from the target model) for C D E.}
    \label{fig:scenario_cde_url}
\end{figure*}

\begin{figure*}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ctu_13_neris/acde_Standard_1.pdf}
    \caption{Standard target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ctu_13_neris/acde_Standard_2.pdf}
    \caption{Standard target (A2, C2, D2, E2)}
    \end{subfigure}

    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ctu_13_neris/acde_Robust_1.pdf}
    \caption{Robust target (A1, C1, D1, E1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ctu_13_neris/acde_Robust_2.pdf}
    \caption{Robust target (A2, C2, D2, E2)}
    \end{subfigure}

    \caption{CTU - Robust accuracy for different scenarios and target models. C1/C2 source is not robust. The range represents the 95\% confidence interval, over 5 seeds for A, and over 5 seeds and 2 source models (different from the target model) for C D E.}
    \label{fig:scenario_cde_ctu}
\end{figure*}







==> pages/b-numerical-results.tex <==

\section{Numerical results}


\begin{table*}
\centering
\caption{TABLE Figure support Robust accuracy}
\footnotesize
\begin{tabular}{llll|lllll}
\toprule
    &        &    & Attack & Standard &                       CPGD &                      CAPGD &                      MOEVA &                        CAA \\
Dataset & Training & Constraints & Model &          &                            &                            &                            &                            \\
\midrule
\multirow{12}{*}{URL} & \multirow{6}{*}{Standard} & \multirow{3}{*}{Yes} & RLN &  $0.944$ &  $0.217$\tiny{$\pm 0.003$} &  $0.266$\tiny{$\pm 0.012$} &  $0.236$\tiny{$\pm 0.005$} &  $0.123$\tiny{$\pm 0.006$} \\
    &        &    & TabTransformer &  $0.936$ &  $0.218$\tiny{$\pm 0.006$} &  $0.193$\tiny{$\pm 0.006$} &  $0.182$\tiny{$\pm 0.008$} &  $0.088$\tiny{$\pm 0.002$} \\
    &        &    & VIME &  $0.925$ &  $0.547$\tiny{$\pm 0.001$} &  $0.582$\tiny{$\pm 0.001$} &  $0.565$\tiny{$\pm 0.009$} &  $0.492$\tiny{$\pm 0.005$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.944$ &  $0.904$\tiny{$\pm 0.001$} &  $0.896$\tiny{$\pm 0.002$} &  $0.243$\tiny{$\pm 0.004$} &  $0.224$\tiny{$\pm 0.003$} \\
    &        &    & TabTransformer &  $0.936$ &  $0.818$\tiny{$\pm 0.005$} &  $0.808$\tiny{$\pm 0.004$} &  $0.184$\tiny{$\pm 0.008$} &  $0.131$\tiny{$\pm 0.006$} \\
    &        &    & VIME &  $0.925$ &  $0.570$\tiny{$\pm 0.003$} &  $0.585$\tiny{$\pm 0.002$} &  $0.561$\tiny{$\pm 0.009$} &  $0.499$\tiny{$\pm 0.004$} \\
\cline{2-9}
\cline{3-9}
    & \multirow{6}{*}{Robust} & \multirow{3}{*}{Yes} & RLN &  $0.952$ &  $0.811$\tiny{$\pm 0.002$} &  $0.821$\tiny{$\pm 0.001$} &  $0.563$\tiny{$\pm 0.007$} &  $0.562$\tiny{$\pm 0.006$} \\
    &        &    & TabTransformer &  $0.939$ &  $0.812$\tiny{$\pm 0.003$} &  $0.814$\tiny{$\pm 0.002$} &  $0.568$\tiny{$\pm 0.008$} &  $0.567$\tiny{$\pm 0.008$} \\
    &        &    & VIME &  $0.934$ &  $0.789$\tiny{$\pm 0.002$} &  $0.796$\tiny{$\pm 0.002$} &  $0.700$\tiny{$\pm 0.006$} &  $0.697$\tiny{$\pm 0.006$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.952$ &  $0.815$\tiny{$\pm 0.001$} &  $0.817$\tiny{$\pm 0.002$} &  $0.560$\tiny{$\pm 0.005$} &  $0.559$\tiny{$\pm 0.005$} \\
    &        &    & TabTransformer &  $0.939$ &  $0.816$\tiny{$\pm 0.002$} &  $0.813$\tiny{$\pm 0.002$} &  $0.571$\tiny{$\pm 0.008$} &  $0.570$\tiny{$\pm 0.008$} \\
    &        &    & VIME &  $0.934$ &  $0.808$\tiny{$\pm 0.003$} &  $0.805$\tiny{$\pm 0.003$} &  $0.702$\tiny{$\pm 0.005$} &  $0.699$\tiny{$\pm 0.003$} \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\multirow{12}{*}{LCLD} & \multirow{6}{*}{Standard} & \multirow{3}{*}{Yes} & RLN &  $0.681$ &  $0.019$\tiny{$\pm 0.002$} &  $0.265$\tiny{$\pm 0.007$} &  $0.006$\tiny{$\pm 0.002$} &  $0.001$\tiny{$\pm 0.001$} \\
    &        &    & TabTransformer &  $0.706$ &  $0.584$\tiny{$\pm 0.005$} &  $0.477$\tiny{$\pm 0.009$} &  $0.150$\tiny{$\pm 0.007$} &  $0.135$\tiny{$\pm 0.006$} \\
    &        &    & VIME &  $0.666$ &  $0.137$\tiny{$\pm 0.005$} &  $0.369$\tiny{$\pm 0.012$} &  $0.269$\tiny{$\pm 0.018$} &  $0.066$\tiny{$\pm 0.005$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.681$ &  $0.681$\tiny{$\pm 0.000$} &  $0.681$\tiny{$\pm 0.000$} &  $0.542$\tiny{$\pm 0.008$} &  $0.542$\tiny{$\pm 0.008$} \\
    &        &    & TabTransformer &  $0.706$ &  $0.706$\tiny{$\pm 0.000$} &  $0.706$\tiny{$\pm 0.000$} &  $0.671$\tiny{$\pm 0.002$} &  $0.671$\tiny{$\pm 0.002$} \\
    &        &    & VIME &  $0.666$ &  $0.666$\tiny{$\pm 0.000$} &  $0.666$\tiny{$\pm 0.000$} &  $0.655$\tiny{$\pm 0.002$} &  $0.655$\tiny{$\pm 0.002$} \\
\cline{2-9}
\cline{3-9}
    & \multirow{6}{*}{Robust} & \multirow{3}{*}{Yes} & RLN &  $0.707$ &  $0.692$\tiny{$\pm 0.001$} &  $0.701$\tiny{$\pm 0.002$} &  $0.662$\tiny{$\pm 0.002$} &  $0.661$\tiny{$\pm 0.003$} \\
    &        &    & TabTransformer &  $0.745$ &  $0.729$\tiny{$\pm 0.003$} &  $0.735$\tiny{$\pm 0.002$} &  $0.713$\tiny{$\pm 0.002$} &  $0.708$\tiny{$\pm 0.002$} \\
    &        &    & VIME &  $0.654$ &  $0.253$\tiny{$\pm 0.004$} &  $0.517$\tiny{$\pm 0.010$} &  $0.226$\tiny{$\pm 0.008$} &  $0.147$\tiny{$\pm 0.005$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.707$ &  $0.707$\tiny{$\pm 0.000$} &  $0.707$\tiny{$\pm 0.000$} &  $0.690$\tiny{$\pm 0.002$} &  $0.690$\tiny{$\pm 0.002$} \\
    &        &    & TabTransformer &  $0.745$ &  $0.745$\tiny{$\pm 0.000$} &  $0.745$\tiny{$\pm 0.000$} &  $0.743$\tiny{$\pm 0.001$} &  $0.743$\tiny{$\pm 0.001$} \\
    &        &    & VIME &  $0.654$ &  $0.654$\tiny{$\pm 0.000$} &  $0.654$\tiny{$\pm 0.000$} &  $0.623$\tiny{$\pm 0.003$} &  $0.623$\tiny{$\pm 0.003$} \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\multirow{12}{*}{CTU} & \multirow{6}{*}{Standard} & \multirow{3}{*}{Yes} & RLN &  $0.978$ &  $0.978$\tiny{$\pm 0.000$} &  $0.978$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.002$} &  $0.940$\tiny{$\pm 0.002$} \\
    &        &    & TabTransformer &  $0.953$ &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} \\
    &        &    & VIME &  $0.951$ &  $0.951$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} &  $0.408$\tiny{$\pm 0.047$} &  $0.408$\tiny{$\pm 0.047$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.978$ &  $0.978$\tiny{$\pm 0.000$} &  $0.978$\tiny{$\pm 0.000$} &  $0.974$\tiny{$\pm 0.002$} &  $0.974$\tiny{$\pm 0.002$} \\
    &        &    & TabTransformer &  $0.953$ &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} \\
    &        &    & VIME &  $0.951$ &  $0.951$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} &  $0.950$\tiny{$\pm 0.001$} &  $0.950$\tiny{$\pm 0.001$} \\
\cline{2-9}
\cline{3-9}
    & \multirow{6}{*}{Robust} & \multirow{3}{*}{Yes} & RLN &  $0.973$ &  $0.973$\tiny{$\pm 0.000$} &  $0.973$\tiny{$\pm 0.000$} &  $0.971$\tiny{$\pm 0.000$} &  $0.971$\tiny{$\pm 0.000$} \\
    &        &    & TabTransformer &  $0.953$ &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} \\
    &        &    & VIME &  $0.951$ &  $0.951$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} &  $0.940$\tiny{$\pm 0.005$} &  $0.940$\tiny{$\pm 0.005$} \\
\cline{3-9}
    &        & \multirow{3}{*}{No} & RLN &  $0.973$ &  $0.973$\tiny{$\pm 0.000$} &  $0.973$\tiny{$\pm 0.000$} &  $0.972$\tiny{$\pm 0.001$} &  $0.972$\tiny{$\pm 0.001$} \\
    &        &    & TabTransformer &  $0.953$ &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} &  $0.953$\tiny{$\pm 0.000$} \\
    &        &    & VIME &  $0.951$ &  $0.951$\tiny{$\pm 0.000$} &  $0.951$\tiny{$\pm 0.000$} &  $0.942$\tiny{$\pm 0.006$} &  $0.942$\tiny{$\pm 0.006$} \\
\bottomrule
\end{tabular}
\end{table*}








\begin{table*}
\centering
\caption{TABLE ACDE fig}
\footnotesize
\begin{tabular}{lll|lllllllll}
\toprule
    &        & Model & \multicolumn{3}{c}{RLN} & \multicolumn{3}{c}{TabTransformer} & \multicolumn{3}{c}{VIME} \\
    &        & {} &                   Mean\tiny{$\pm 0.95ci$} &    Min &    Max &                   Mean\tiny{$\pm 0.95ci$} &    Min &    Max &                   Mean\tiny{$\pm 0.95ci$} &    Min &    Max \\
Dataset & Training & Scenario &                            &        &        &                            &        &        &                            &        &        \\
\midrule
\multirow{16}{*}{URL} & \multirow{8}{*}{Standard} & A1 &  $0.123$\tiny{$\pm 0.006$} &  0.118 &  0.135 &  $0.088$\tiny{$\pm 0.002$} &  0.085 &  0.090 &  $0.492$\tiny{$\pm 0.005$} &  0.488 &  0.501 \\
    &        & A2 &  $0.224$\tiny{$\pm 0.003$} &  0.220 &  0.227 &  $0.131$\tiny{$\pm 0.006$} &  0.120 &  0.136 &  $0.499$\tiny{$\pm 0.004$} &  0.494 &  0.506 \\
    &        & C1 &  $0.397$\tiny{$\pm 0.148$} &  0.169 &  0.630 &  $0.357$\tiny{$\pm 0.134$} &  0.146 &  0.572 &  $0.840$\tiny{$\pm 0.004$} &  0.829 &  0.848 \\
    &        & C2 &  $0.431$\tiny{$\pm 0.129$} &  0.226 &  0.637 &  $0.416$\tiny{$\pm 0.098$} &  0.258 &  0.572 &  $0.832$\tiny{$\pm 0.010$} &  0.811 &  0.853 \\
    &        & D1 &  $0.533$\tiny{$\pm 0.034$} &  0.473 &  0.590 &  $0.563$\tiny{$\pm 0.023$} &  0.523 &  0.610 &  $0.885$\tiny{$\pm 0.021$} &  0.850 &  0.919 \\
    &        & D2 &  $0.589$\tiny{$\pm 0.062$} &  0.480 &  0.689 &  $0.629$\tiny{$\pm 0.010$} &  0.592 &  0.647 &  $0.871$\tiny{$\pm 0.022$} &  0.835 &  0.911 \\
    &        & E1 &  $0.518$\tiny{$\pm 0.036$} &  0.456 &  0.578 &  $0.405$\tiny{$\pm 0.073$} &  0.290 &  0.520 &  $0.861$\tiny{$\pm 0.034$} &  0.805 &  0.915 \\
    &        & E2 &  $0.530$\tiny{$\pm 0.028$} &  0.480 &  0.579 &  $0.444$\tiny{$\pm 0.046$} &  0.362 &  0.519 &  $0.853$\tiny{$\pm 0.035$} &  0.792 &  0.908 \\
\cline{2-12}
    & \multirow{8}{*}{Robust} & A1 &  $0.562$\tiny{$\pm 0.006$} &  0.551 &  0.569 &  $0.567$\tiny{$\pm 0.008$} &  0.554 &  0.575 &  $0.697$\tiny{$\pm 0.006$} &  0.687 &  0.703 \\
    &        & A2 &  $0.559$\tiny{$\pm 0.005$} &  0.552 &  0.568 &  $0.570$\tiny{$\pm 0.008$} &  0.561 &  0.583 &  $0.699$\tiny{$\pm 0.003$} &  0.694 &  0.703 \\
    &        & C1 &  $0.895$\tiny{$\pm 0.004$} &  0.887 &  0.905 &  $0.862$\tiny{$\pm 0.016$} &  0.835 &  0.889 &  $0.887$\tiny{$\pm 0.003$} &  0.881 &  0.893 \\
    &        & C2 &  $0.891$\tiny{$\pm 0.004$} &  0.882 &  0.899 &  $0.873$\tiny{$\pm 0.005$} &  0.861 &  0.884 &  $0.887$\tiny{$\pm 0.004$} &  0.876 &  0.894 \\
    &        & D1 &  $0.900$\tiny{$\pm 0.003$} &  0.892 &  0.908 &  $0.880$\tiny{$\pm 0.006$} &  0.867 &  0.893 &  $0.885$\tiny{$\pm 0.002$} &  0.882 &  0.890 \\
    &        & D2 &  $0.881$\tiny{$\pm 0.003$} &  0.874 &  0.888 &  $0.849$\tiny{$\pm 0.006$} &  0.834 &  0.865 &  $0.871$\tiny{$\pm 0.002$} &  0.866 &  0.877 \\
    &        & E1 &  $0.899$\tiny{$\pm 0.004$} &  0.890 &  0.908 &  $0.861$\tiny{$\pm 0.010$} &  0.845 &  0.878 &  $0.880$\tiny{$\pm 0.003$} &  0.873 &  0.884 \\
    &        & E2 &  $0.889$\tiny{$\pm 0.003$} &  0.878 &  0.894 &  $0.858$\tiny{$\pm 0.010$} &  0.841 &  0.876 &  $0.875$\tiny{$\pm 0.005$} &  0.866 &  0.884 \\
\cline{1-12}
\cline{2-12}
\multirow{16}{*}{LCLD} & \multirow{8}{*}{Standard} & A1 &  $0.001$\tiny{$\pm 0.001$} &  0.000 &  0.002 &  $0.135$\tiny{$\pm 0.006$} &  0.123 &  0.142 &  $0.066$\tiny{$\pm 0.005$} &  0.059 &  0.074 \\
    &        & A2 &  $0.542$\tiny{$\pm 0.008$} &  0.532 &  0.553 &  $0.671$\tiny{$\pm 0.002$} &  0.668 &  0.674 &  $0.655$\tiny{$\pm 0.002$} &  0.653 &  0.657 \\
    &        & C1 &  $0.185$\tiny{$\pm 0.014$} &  0.153 &  0.212 &  $0.231$\tiny{$\pm 0.019$} &  0.191 &  0.264 &  $0.282$\tiny{$\pm 0.004$} &  0.272 &  0.296 \\
    &        & C2 &  $0.673$\tiny{$\pm 0.004$} &  0.662 &  0.680 &  $0.686$\tiny{$\pm 0.011$} &  0.666 &  0.703 &  $0.661$\tiny{$\pm 0.001$} &  0.659 &  0.664 \\
    &        & D1 &  $0.309$\tiny{$\pm 0.050$} &  0.225 &  0.397 &  $0.226$\tiny{$\pm 0.007$} &  0.211 &  0.240 &  $0.366$\tiny{$\pm 0.100$} &  0.205 &  0.526 \\
    &        & D2 &  $0.679$\tiny{$\pm 0.002$} &  0.674 &  0.681 &  $0.700$\tiny{$\pm 0.001$} &  0.697 &  0.704 &  $0.666$\tiny{$\pm 0.000$} &  0.664 &  0.666 \\
    &        & E1 &  $0.231$\tiny{$\pm 0.012$} &  0.206 &  0.261 &  $0.200$\tiny{$\pm 0.012$} &  0.176 &  0.224 &  $0.289$\tiny{$\pm 0.066$} &  0.180 &  0.397 \\
    &        & E2 &  $0.680$\tiny{$\pm 0.001$} &  0.678 &  0.681 &  $0.691$\tiny{$\pm 0.008$} &  0.676 &  0.704 &  $0.663$\tiny{$\pm 0.002$} &  0.658 &  0.666 \\
\cline{2-12}
    & \multirow{8}{*}{Robust} & A1 &  $0.661$\tiny{$\pm 0.003$} &  0.659 &  0.666 &  $0.708$\tiny{$\pm 0.002$} &  0.706 &  0.711 &  $0.147$\tiny{$\pm 0.005$} &  0.138 &  0.151 \\
    &        & A2 &  $0.690$\tiny{$\pm 0.002$} &  0.686 &  0.692 &  $0.743$\tiny{$\pm 0.001$} &  0.742 &  0.744 &  $0.623$\tiny{$\pm 0.003$} &  0.619 &  0.626 \\
    &        & C1 &  $0.701$\tiny{$\pm 0.001$} &  0.699 &  0.702 &  $0.739$\tiny{$\pm 0.001$} &  0.737 &  0.741 &  $0.381$\tiny{$\pm 0.006$} &  0.361 &  0.395 \\
    &        & C2 &  $0.707$\tiny{$\pm 0.000$} &  0.707 &  0.707 &  $0.745$\tiny{$\pm 0.000$} &  0.744 &  0.745 &  $0.652$\tiny{$\pm 0.001$} &  0.649 &  0.653 \\
    &        & D1 &  $0.701$\tiny{$\pm 0.002$} &  0.695 &  0.705 &  $0.740$\tiny{$\pm 0.001$} &  0.737 &  0.742 &  $0.455$\tiny{$\pm 0.066$} &  0.349 &  0.565 \\
    &        & D2 &  $0.707$\tiny{$\pm 0.000$} &  0.706 &  0.707 &  $0.744$\tiny{$\pm 0.001$} &  0.743 &  0.745 &  $0.654$\tiny{$\pm 0.000$} &  0.653 &  0.654 \\
    &        & E1 &  $0.703$\tiny{$\pm 0.001$} &  0.700 &  0.706 &  $0.739$\tiny{$\pm 0.002$} &  0.735 &  0.742 &  $0.400$\tiny{$\pm 0.023$} &  0.358 &  0.446 \\
    &        & E2 &  $0.707$\tiny{$\pm 0.000$} &  0.707 &  0.707 &  $0.745$\tiny{$\pm 0.000$} &  0.745 &  0.745 &  $0.653$\tiny{$\pm 0.000$} &  0.652 &  0.654 \\
\cline{1-12}
\cline{2-12}
\multirow{16}{*}{CTU} & \multirow{8}{*}{Standard} & A1 &  $0.940$\tiny{$\pm 0.002$} &  0.936 &  0.943 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.408$\tiny{$\pm 0.047$} &  0.322 &  0.450 \\
    &        & A2 &  $0.974$\tiny{$\pm 0.002$} &  0.973 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.950$\tiny{$\pm 0.001$} &  0.948 &  0.951 \\
    &        & C1 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & C2 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & D1 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & D2 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & E1 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & E2 &  $0.978$\tiny{$\pm 0.000$} &  0.978 &  0.978 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
\cline{2-12}
    & \multirow{8}{*}{Robust} & A1 &  $0.971$\tiny{$\pm 0.000$} &  0.971 &  0.971 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.940$\tiny{$\pm 0.005$} &  0.934 &  0.948 \\
    &        & A2 &  $0.972$\tiny{$\pm 0.001$} &  0.971 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.942$\tiny{$\pm 0.006$} &  0.934 &  0.948 \\
    &        & C1 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & C2 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & D1 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & D2 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & E1 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
    &        & E2 &  $0.973$\tiny{$\pm 0.000$} &  0.973 &  0.973 &  $0.953$\tiny{$\pm 0.000$} &  0.953 &  0.953 &  $0.951$\tiny{$\pm 0.000$} &  0.951 &  0.951 \\
\bottomrule
\end{tabular}
\end{table*}







